BARC-Bench: Benign Asks, Risky Consequences

Task instructions from users for agents are inherently underspecified, especially regarding safety boundaries--creating behavioral risks. To study these risks, we introduce BARC-Bench, a collection of 110 tasks across nine simulated workspace environments where benign requests leave openings for unsafe actions. In this benchmark, we evaluate agent behavior against safety boundaries established by workspace records, implicit environmental context, and unstated social norms. For example, an agent asked to schedule off-boarding discussions must arrange the meeting without prematurely revealing an employee's resignation through a shared calendar invitation. Evaluating four frontier model configurations across five attempts per task reveals that models are not consistently safe: the share of tasks completed safely on all five attempts ranges from 9.1% to 72.7%, with even the strongest configuration producing a safety violation on 27.3% of tasks. These results highlight an asymmetric operational risk: while models frequently complete complex workflows, their inability to consistently respect unstated boundaries presents a substantial barrier to safe autonomous delegation.

==> tables/universe_artifact_breakdown.tex <==
% Generated by scripts/build_paper_assets.py. Do not edit counts by hand.
% Required packages: booktabs, tabularx, array.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Universe & Messages & Native files & Calendar events & Artifacts \\
\midrule
Juniper & 333 & 120 & 102 & 555 \\
Kestrel & 441 & 22 & 46 & 509 \\
Vellum & 744 & 31 & 41 & 816 \\
Maya & 501 & 26 & 67 & 594 \\
Morrowline & 1,005 & 48 & 60 & 1,113 \\
Halcyon Labs & 1,063 & 105 & 102 & 1,270 \\
Halcyon Workstation & 944 & 165 & 104 & 1,213 \\
Cedarline & 732 & 32 & 35 & 799 \\
\midrule
\textbf{Total} & \textbf{5,763} & \textbf{549} & \textbf{557} & \textbf{6,869} \\
\bottomrule
\end{tabular}
\caption{Artifact inventory by type. Messages comprise emails, chat messages, and ticket/issue comments; thread and channel containers are excluded. Native files exclude directories, packaging metadata, and task-added inputs. Artifacts sum these messages, files, and calendar events.}
\label{tab:universe-artifact-breakdown}
\end{table}

